How Does User Behavior Evolve During Exploratory Visual Analysis?

Exploratory visual analysis (EVA) is an essential stage of the data science pipeline, where users often lack clear analysis goals at the start and iteratively refine them as they learn more about their data. Accurate models of users' exploration behavior are becoming increasingly vital to developing responsive and personalized tools for exploratory visual analysis. Yet we observe a discrepancy between the static view of human exploration behavior adopted by many computational models versus the dynamic nature of EVA. In this paper, we explore potential parallels between the evolution of users' interactions with visualization tools during data exploration and assumptions made in popular online learning techniques. Through a series of empirical analyses, we seek to answer the question: how might users' exploration behavior evolve in response to what they have learned from the data during EVA? We present our findings and discuss their implications for the future of user modeling for system design.

==> 2_2_user_studies_overview.tex <==
\subsection{Selected User Studies}
Rather than conducting a separate user study to collect data, we leverage publicly shared user studies from researchers \cite{battle2019characterizing,liu2014effects, battle2016dynamic} who have already conducted influential studies in this space. 
Leveraging these studies (\autoref{tab:user_study_table}) lets us analyze diverse real-life data analysis tasks that vary across different facets of data exploration.   

In the \textbf{Tableau user study}, the users used Tableau\cite{Tableau} to explore three different datasets to simulate large-scale data analysis with appropriate complexity and size.
%including flight performance, weather, and wildlife strikes,
Battle et al. designed a diverse set of focused tasks, varying in data requirements, and a goal-directed open-ended task that reflects real-life data analysis tasks to investigate users' analytic behavior in fine detail\cite{battle2019characterizing}.

In the {\bf ForeCache user study}, users interactively explore a 2D map of the US.
% The 2D map is created on a white canvas that clearly outlines all US states.
It uses different shades of blue to indicate the amount of snow cover, with darker shades representing areas with higher snow accumulation. Users are required to locate and capture three screenshots from the regions with the most extensive snow cover\cite{battle2016dynamic}.
%with various geographical information : added

The \textbf{imMens user study} had participants explored flight performance and travel history data to uncover interesting insights, such as unexpected events, data abnormalities, or confirmations of common knowledge and intuition. 
Each participant had 30 minutes to examine a single dataset and could terminate the session early if they felt there was nothing noteworthy to report. \cite{liu2014effects} 
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
%------------------------------------------------------------

% We also want to observe whether users behave differently while interacting with different visualizations. For instance, in the completely open-ended task, users prefer to interact with spatial visualization than temporal visualization, which is evident in \autoref{fig: time_spent_tableau}.

%---------------------
% \subsubsection{Correctness driven}
% In some tasks, users might be required to provide verification of their findings. For instance, they Users might learn to perform the tasks with correctness verification differently than the one without this step.
% Also, The tasks that require verification might induce a different learning scheme The verification step 

%-------------------------------------------
% \subsubsection{Correctness driven}
% From the \textit{'Correctness driven'} row in \autoref{tab:user_study_high_level}, we observe that verification of findings weren't required for participants in open-ended tasks (\textit{User study 1 and User study 3:T4}). However, in the focused tasks users could verify their answers to some extent. 
% In \textit{User study 1}, participants worked with a travelers' check-in dataset and had diverse intents. Some wanted to identify popular tourist locations, while others focused on determining the best time of the year to travel, and some were interested in analyzing users' sleep and eating patterns. The unique areas of focus and ordering among participants in open-ended tasks indicate individualism, and we demonstrate in \autoref{subsec: iMens_nonstationarity} that their exploration behavior varies while examining different areas.

\begin{comment}
\leilani{I would introduce the spectrum of possible tasks here, which will act as an outline for the rest of the section. My survey of exploratory visual analysis could be a good anchor for the overview~\cite{battle2019characterizing}. This paper talks about how exploration can be focused, goal-directed, or even fully open-ended.}
\leilani{I see \autoref{tab:user_study_high_level} contains more variables than are introduced at the beginning of this section. For this table, I would either trim it to match the content of this section, or expand the section to consider more of the high-level variables.}
\end{comment}

\begin{comment}
\leilani{This paragraph seems to hint at trade-offs in decreasing task structure and increasing "noise" (basically variance across individuals' behaviors). It would be nice to think about what other high-level themes there are surrounding task type, name these themes, and introduce them early in the section. Rather than themes, we could also refer to them as "considerations" (task open-endedness, user experience, etc.). Then, these themes/considerations could be paragraph or section headers to give this section more structure.}
\end{comment}

\begin{comment}
\leilani{I don't see \autoref{tab:user_study_information} as playing a significant role in this section. I see it as providing details reviewers will probably ask for but could be looked up in the original papers. If we want to introduce an overview of all studies just to provide some details, we may want a separate subsection for that.}
\end{comment}

==> 2_3_user_study_characteristics.tex <==
\vspace{-3mm}
\subsection{Characteristics captured by selected studies}
Rather than conducting a separate user study to collect data, we leverage publicly shared user studies from researchers \cite{battle2019characterizing,liu2014effects, battle2016dynamic} who have already conducted influential studies in this space. 
Leveraging these studies (\autoref{tab:user_study_table}) lets us analyze diverse real-life data analysis tasks that vary across different facets of data exploration. 
We propose that our selected studies capture different characteristics of exploration tasks and may serve as a key factor in evaluating the efficacy of our user-learning models. 
% For instance, similar user-learning schemes may attain contrasting performances depending on how well-defined the objectives of their tasks are. 

\subsubsection{Open-endedness:}
\label{sec:characteristic_openendedness}
In the \textit{imMens user study}, participants explore three datasets with the vague goal of finding something \textit{interesting}, without prior intent or hypotheses, i.e., doing completely open-ended task. 
We employ the \textit{Tableau user study: T4} to analyze users' learning behavior in the goal-directed open-ended task.

\noindent
\textit{Example:} For one of the tasks in the \textit{Tableau user study: T4}, users were required to identify potential airports for Delta airlines to expand its operations using the flight performance dataset. Unlike in completely open-ended tasks, users had to conduct a controlled exploration to learn about relevant entities to achieve this goal. 

% Rather than exploring the dataset without intent, in goal-directed open-ended tasks the user must conduct a controlled exploration to search for entities leading to successful airports where Delta is not operating. 
In the focused tasks \textit{(e.g., ForeCache user study, Tableau user study [T1, T2, T3])}, the participants have a clear idea of what entities to search for or what data area to focus into. After they explore the data to locate them, they can exploit those to find the desired information. On the other hand, in open-ended tasks, users may form intents and hypotheses more than their focused counterparts to find the desired information. If their hypothesis fails, users adapt their strategy and start again to form a new hypothesis. Our empirical analysis in this paper shows that as data exploration progresses, these decision-making policies change.

 %-------------------------------------------
\noindent
\subsubsection{Prior experience}
The \textit{ForeCache user study} provided users with the opportunity to become familiar with the dataset and interface, while in the other two studies, users started exploration with no prior knowledge. This diversity in the selected dataset allows us to examine the impact of prior experience on user learning.

%-------------------------------------------
\noindent
\subsubsection{Time restriction}
Our user study selection has time restriction ranging from no restriction to a 30-minute limit. 
%spans a diverse spectrum of time restrictions, ranging
\textit{Forecache user study} did not impose a time restriction as the task instructions were clearly defined, and required less time to complete the task. In contrast, the completely open-ended nature of the \textit{imMens user study} necessitated a cut-off threshold, as there could be \textit{numerous insights} that users may discover with an unbounded time frame.

%-------------------------------------------
\noindent
\subsubsection{Cognitive load by the system interfaces:}
Our user studies involved systems with diverse ways of presenting information to facilitate interactive data exploration (\autoref{tab:user_study_high_level}). ForeCache displayed snow cover on a 2D map with similar functionality to Google maps.
imMens automatically generated visual summaries of large multi-dimensional datasets and allowed users to perform visual queries using minimal operations. 
In contrast, Tableau was a more complex system where users had to select data areas to visualize, filter raw data, choose easy-to-interpret visualizations, and numerous available operations facilitating exploration. 
It made our process of modeling users' decision-making problems challenging,  requiring multiple models to represent them.


==> 2_3_user_study_characteristics_new.tex <==
\vspace{-3mm}
\subsection{Characteristics captured by selected studies}
Rather than conducting a separate user study to collect data, we leverage publicly shared user studies from researchers \cite{battle2019characterizing,liu2014effects, battle2016dynamic} who have already conducted influential studies in this space. 
Leveraging these studies (\autoref{tab:user_study_table}) lets us analyze diverse real-life data analysis tasks that vary across different facets of data exploration.

We propose that our selected studies capture different characteristics (\autoref{tab:user_study_high_level}) of exploration tasks and serve as a key factor in evaluating the efficacy of our user-learning models. 
For instance, similar user-learning schemes may attain contrasting performances depending on how well-defined the objectives of their tasks are. 

\noindent
\textit{Example:} In open-ended tasks, users may form intents and hypotheses more than their focused counterparts. If their hypothesis fails, users adapt their strategy and restart with a new hypothesis to find the desired information. Our empirical analysis shows that as data exploration progresses, these decision-making policies change.

% \noindent
% \textit{Example:} For one of the tasks in the \textit{Tableau user study: T4}, users were required to identify potential airports for Delta airlines to expand its operations using the flight performance dataset. 
% % Unlike in completely open-ended tasks, users had to conduct a controlled exploration to learn about relevant entities to achieve this goal. 
% Rather than exploring the dataset without intent, in goal-directed open-ended tasks the user must conduct a controlled exploration to search for entities leading to successful airports where Delta is not operating. 

% \textit{Forecache user study} did not impose a time restriction as the task instructions were clearly defined, and required less time to complete the task. In contrast, the completely open-ended nature of the \textit{imMens user study} necessitated a cut-off threshold, as there could be \textit{numerous insights} that users may discover with an unbounded time frame.


==> 3_2_tableau_non_stationarity.tex <==
\vspace{-2mm}
% \subsubsection{Mann-Whitney U test for non-stationarity analysis:}
\subsubsection{Non-stationarity 50-50 Split:}
\label{sec: man_whitney}
First, we divide each participant's exploration session into two stages for each task (initial and later exploration). 
Next, we generate the exploration policies, i.e., the probability of using the same attributes throughout a task. 
% Finally, we use the Mann-Whitney U test \cite{mcknight2010mann, mann1945nonparametric} to determine the non-stationarity of a user's exploration policy.
Finally, to evaluate the non-stationarity of user strategies, we use the Mann-Whitney U test\cite{mcknight2010mann, mann1945nonparametric}, which is a non-parametric test used to test whether two samples are likely to derive from the same population (i.e., the two stages have the same strategy). If we see a significant deviation in users' exploration policy (i.e., attribute preferences) in the later stages of exploration compared to their initial, it means the user adopted a non-stationary exploration strategy. 

Importantly, we conduct non-stationarity tests on individual attribute preferences rather than considering the group of attributes used in each interaction.
The reason is to overcome the scenario where a user has a fixed preference for some attributes (e.g., \{A, B, C\}). 
While keeping a set fixed, she adds and removes attributes from the dataset to modify her selection(e.g., \{A, B, C, D, E\}). 
For example, she may add \textbf{D} (\{A, B, C, {\bf D}\}) and subsequently drop it (\{A, B, C\}), or she may explore \textbf{E} by adding it (\{A, B, C, {\bf E}\}) and then dropping it (\{A, B, C\}).
A non-stationarity test based on attribute groups will overlook her stationary preference of the fixed set.
As a result, if the number of non-stationary attributes is more than 50\%, we consider the exploration policy non-stationary.
  

% \leilani{This terminology is not consistent with the terminology in Section 2.2.}
\begin{comment}
\textbf{Mann-Whitney U-test:}
Mann-Whitney U-test is a non-parametric test that allows us to check whether two distributions are from the same population. Furthermore, we do not need to make any assumptions on the sample size and actual distribution \textit{(e.g. t-test requires large sample size and normal distribution)}. We proceed with the statistical tests in the following way: we focus on two mutually exclusive time intervals of a user's activity. Two series are generated from those two intervals, each containing the probability of making certain decisions at each interaction. Using the Mann-Whitney U-test statistic \textit{(p-value)}, we examine whether the following null hypothesis gets rejected.
\textit{Null hypothesis: The two groups under consideration have the
same distribution, i.e., a user's likelihood of making a specific decision did not change significantly (stationary)}
\end{comment}
\vspace{-3mm}
\begin{figure}[!htbp]
\centering
% \includegraphics[scale=0.44]{figures/TableauNonStationary.png}
\includegraphics[scale=0.75]{figures/final2.pdf}
\vspace{-5mm}
\caption{Stationarity test result in Tableau user study}
% \caption{In the \textit{focused tasks} (T1-T3), users exhibit mainly \textit{stationary} behavior, whereas in the goal-directed task (T4), both types of behavior are observed. 
% }
\vspace{-5mm}
\label{fig: tableau_non_stationary}
\end{figure}
\noindent
% \subsubsection{Our observation from test results:}
% We will use the analysis tasks (shown in \autoref{tab:tableau-table})from the Weather dataset for reference. 
% In our observation of users' exploration behavior in T4 (which doesn't contain any hints), we see the majority of the users selecting attributes that they learned in the focused task rather than exploring new attributes.  
% Now, this exploration behavior is caused by the high correlation of this analysis task with the prior focused tasks. 
% However, few users are adventurous and explored new attributes to enhance their answers.

\subsubsection{Analyzing Non-stationarity Test Results:}
\label{sec: tableau_non_stationarity}
\autoref{fig: tableau_non_stationary} shows that users mainly adopt stationary exploration policies in the focused tasks ($77\%$ of the users), but for the goal-directed tasks, we see a mix of stationary ($53\%$) and non-stationary ($47\%$) policies depending on whether new attributes are required to complete them.

This result matches our observation in the focused tasks: most users only explore the attributes stated in the task prompt without changing attribute preferences.
For instance, in $T1$ \& $T2$, users try different visualizations in Tableau using the \textit{stated} attributes (e.g., [Date] in \autoref{tab:tableau-table}).
Occasionally, users explore a couple more attributes, but most of the time, they have \textit{a fixed attribute preference}. 
% After reviewing the visualizations, they answer the task.

On the other hand, goal-directed tasks require participants to identify necessary attributes for task completion, e.g., weather prediction in \autoref{tab:tableau-table}.
Users learn about weather dataset attributes through the completed focused tasks, such as fog, mist, drizzle, temperature, wind, and date.
Some users only explore these data areas and apply different visualizations to predict the weather, adopting a \textit{fixed exploration strategy}.
Yet some users exhibit a more exploratory approach and thoroughly analyze other attributes before making predictions, e.g., precipitation, hail, glaze, state, dust, etc.
Here, users' attribute preferences change more frequently, resulting in a \textit{non-stationary exploration strategy}.

To summarize, we find that a subset of participants in this study seem to change their exploration strategy in response to what they learn as they explore using Tableau. 
Specifically, users do \emph{not} seem to exhibit learning-driven behaviors during the focused tasks but \emph{do} seem to be more learning-driven during goal-directed tasks.

% Investigating users' exploration behavior in this user study, we found that users predominantly adopt a stationary exploration policy during focused tasks. 
% They primarily explore the provided set of attributes, which proves sufficient for task completion.
% But we also observe a few users using this knowledge as a starting point and exploring additional attributes, resulting in a non-stationary exploration policy. 

% \autoref{fig: tableau_non_stationary} shows that $77\%$ of the users adopt a stationary exploration policy in the focused tasks.
% \leilani{Will the reader know that ``stationary policy'' means they do not change their behavior across stages?}

% We utilize the Mann-Whitney U-test for our non-stationarity analysis, splitting user interactions in half.
% Under each task completed by the users, we create a separate series for each attribute, reflecting the probability of its appearance during an interaction. Non-stationarity analysis is then performed on these series to determine whether the user's interest in a particular attribute has waned, leading to its removal from their preferred list.   

% \leilani{what does ``perform visual analytics'' mean? Participants created visualizations in Tableau using the requested attributes and maybe a couple more attributes, reviewed the visualizations, then gave an answer to the tasks...}
% The tasks also do not require them to explore other data areas for success.  

\begin{comment}
On the other hand, goal-directed tasks require participants to identify the attributes necessary for task completion.  
% We can see from (\autoref{fig: tableau_non_stationary}) that in $T4$ tasks, $47\%$ of users adopt non-stationary exploration policies while $53\%$ follow stationary exploration policies.
We observe learning about the data areas in the focused tasks affecting their exploration behavior in $T4$.
Let us consider the analysis tasks from the Weather dataset in \autoref{tab:tableau-table}. The majority of the users select attributes that they learned about in the previous tasks (T1-T3) rather than exploring new attributes during T4.
\leilani{the following sentence is not a complete sentence:} As prior knowledge about attributes \textit{fog, mist, drizzle, temperature, wind, and date} from the focused tasks may be enough for weather prediction.
Thus our experiment result of $75\%$ users adopting a stationary policy while exploring the Weather dataset for $T4$ aligns with our high-level observation.
% the exploration carried out in the focused tasks sufficiently covers the data areas necessary for task $T4$ completion.

Other goal-directed open-ended tasks with wildlife strike and flight performance dataset (details available in \cite{battle2019characterizing}) require exploring new attributes. It influences more users (60\%) to adopt a non-stationary approach.
Users who adopt a stationary strategy assume their initial attribute selection provides adequate evidence to complete the prediction task $T4$.
\end{comment}



% Users who adopt a stationary strategy in their exploration do not venture beyond their focused data area, considering it provided adequate evidence for the prediction tasks.
% This diverse nature of users' exploration behavior is profoundly informative as it portrays the variation in information needs across users and the importance of adapting to individual users' exploration policies to facilitate IDE.
% \leilani{the organization of these descriptions is confusing. I think it's saying that for focused tasks the results are mainly stationary, but for the goal-directed tasks we see a mix of stationary and non-stationary behavior depending on whether new attributes are required to complete the task. We should provide this overview first, then describe the details.}

% \leilani{Also, there should be some easy to find (e.g., bolded) takeaway statement from this subsection, even if all it says is: ``To summarize, we find that a subset of participants from the Battle et al. study seem to change their exploration strategy in response to what they learn as they explore using Tableau Desktop. Specifically, users do \emph{not} seem to exhibit learning-driven behaviors during the focused tasks but \emph{do} seem to be more learning driven during goal-directed tasks.''}

% Half of the users were content with relating their learned attributes to the information needs in T4; the other half were adventurous and wanted to explore more attributes \textit{(which weren't in the recommended set of attributes, e.g., precipitation, snow, thunder, smoke, etc.)} before concluding.

% The users with non-stationary decision-making policy tried out different attributes and often added or removed attributes from their preference list.

% \leilani{This subsection should have clear takeaways that naturally lead to the next sub-section (i.e., the next stage of the analysis). What are the major takeaways for the non-stationary analysis that inform the modeling of user learning? They are not clear. See the HILDA paper for example framing.}


==> 3_2_tableau_stationarity.tex <==
\subsection{Modeling users' decision problem}

\leilani{There needs to be a bit more of a story in the beginning explaining why we are doing this modeling. Please see my edits/suggestions to the HILDA paper for an example. Also, this story should translate through the entire section as well. Papers always tell a story. They do not just relay a list of facts. Why should readers be interested in each part of the story? Why does it matter? Readers need to know upfront, before they read each section and subsection. Otherwise, they may feel compelled to just skip that content. Why read it if there's no explanation to its value?}

\leilani{Also, each paragraph should lead with the key idea behind the paragraph, and ideally end with a connector to the next paragraph (i.e., connect to the next key idea in the story). This is an extreme example, but it should be possible to get the gist of the entire paper just by reading the section headers, sub-section headers, and the first sentence of every paragraph. This property makes the paper ``skimmable''.}

\subsubsection{Users' activities:} 
Users could select any number of \textit{\textbf{attributes}} using Tableau \textit{(from dimension and measure column)}, and add them to a worksheet, which Tableau would use to generate visualizations for easy data comprehension. 
Users could add or remove attributes, filter or aggregate particular attributes, try different visualizations, or start over based on the current screen.

% Due to the nature of the analysis task and the human cognitive load limitations discussed in Section \ref{sec: cognitive}, we observed that users utilized an average of $3.34$ $\approx$ $3$ attributes per interaction. While this "sweet spot" may vary based on the user's preferences or analysis task, it is essential to establish a fixed number to analyze how the users' decision-making process evolves during exploration. Instead of predicting how many attributes a user will use per interaction, we prioritize understanding how their learning behavior changes throughout the exploration session.

\subsubsection{Users' decision problem:}
To analyze user learning behavior during exploration, we examine how their attribute preferences influence their decision-making policies. During each interaction (time-step), \textit{users would decide which set of \textbf{attributes} they should pick to get their desired information.} They can modify the current set by adding or removing one or more attributes (resulting in a new attribute set), which can increase information, ease interpretation. 
Users can also keep using the same set of attributes, then perform data manipulation and visualization change operations. Furthermore, they can reset their progress and start anew.

As mentioned earlier, users received hints on which attributes to focus on during focused analysis tasks. We investigate how closely users followed these hints. Additionally, since users completed T1-T4 sequentially, we are interested in exploring the impact of focused tasks on the goal-directed open-ended tasks. 

\leilani{I highly recommend comparing the story flow of the HILDA paper to this section. This section should have the same story structure/flow as the HILDA paper.}

\begin{figure}[!]
\centering
\includegraphics[scale=0.23]{figures/tableu-ns.png}
\caption{In the \textit{focused tasks} (T1-T3), users exhibit mainly \textit{stationary} behavior, whereas in the goal-directed open-ended task (T4), both types of behavior are observed.}
\label{fig: tableau_non_stationary}
\end{figure}

\subsubsection{Combinatorial Multi-arm bandit (CMAB)}
\label{subsubsection: cmab}
In this variation of the multi-arm bandit (MAB), the user can choose a subset of $n$ arms instead of selecting only one arm per time step, as in the general MAB. 
CMAB presents $n$ variables $X = \{X_1, ..., X_n\}$, where variable $X_i$ can take $K_i$ different values $\chi_i = \{v^{1}_i, ... , v^{K_i}_i\}$. The reward $R : \{\chi_1 \times ... \times \chi_i\} \rightarrow \mathbb{R}$ depends on the values of each of these variables. 
The goal of the problem is to find a vector $V \subseteq \{0, 1\}^n$ representing the subset combination of arms that minimizes the regret in \autoref{eqn: combinatorial_regret}\cite{ontanon2013combinatorial, ontanon2017combinatorial}. \autoref{eqn: combinatorial_regret} presents the regret equation for policy $\pi$, where $x^{t}_1, ..., x^{t}_n$ are the values selected at time step T. 
\begin{equation}
    \rho(\pi, t) = T \mu^* - \sum_{t = 1}^{T} R(x^{t}_1, ..., x^{t}_n)
    \label{eqn: combinatorial_regret}
\end{equation}
Here, $\mu^{*} = \mathbb{E}(R(v^{*}_1, ..., v^{*}_1))$ is the maximum expected reward gained by following the optimal policy $\pi^{*}$.

\subsubsection{Modeling users' decision-problem using CMAB:}
In the \textit{Tableau user study}, users face a sequential decision problem where they select attributes, perform operations, and observe visualizations to extract relevant information. 
The users receive information as a reward, which guides their exploration process. 
\textit{Users focus on a subset of attributes in each time step and examine Tableau-generated visualizations.} Upon operating on them, if a user believes she has extracted the necessary information, she can focus on a different data area for new information or generate new hypotheses. 
It is possible by adding or removing attributes from the current set and resetting to start anew.  
Besides, the user might use the same attribute set to improve or verify their present understanding.

\leilani{I think these paragraphs are out of order, evidenced by the backward reference in the following paragraph. The first thing the reader will want to know are our assumptions regarding how users behave. These assumptions inform the type of model we would use. With an understanding of the assumptions (the preliminaries), then the reader will want to know about the specific model design.}

The decision-making problem we are addressing is akin to the CMAB problem discussed in \autoref{subsubsection: cmab}.
% In the multi-armed bandit setting, a user has N bandits or attributes to choose from, with the user able to pick only one arm at a time. 
The decision-making problem involves users selecting a set of attributes at each interaction. The users focus on finding the optimal subset of attributes that will give them the maximal reward, i.e., leading them to the information asked in the analysis tasks. This is similar to finding the optimal subset of arms in the CMAB setting. 

\subsection{Non-Stationarity analysis}

\leilani{The non-stationary analysis should be introduced before the model assumptions and design, since this motivates the need for modeling learning or not. If users are not learning, then there's no need to model learning. Again, I think the story is out of order and insufficient motivation is being applied.}

\subsubsection{Mann-Whitney U-test:}\label{sec: man_whitney} We use statistical tests to check if users' decision-making policy changes during data exploration. \textbf{Mann-Whitney U-test} is a non-parametric test that allows us to check whether two distributions are from the same population. Furthermore, we do not need to make any assumptions on the sample size and actual distribution \textit{(e.g. t-test requires large sample size and normal distribution)}. We proceed with the statistical tests in the following way: we focus on two mutually exclusive time intervals of a user's activity. Two series are generated from those two intervals, each containing the probability of making certain decisions at each interaction. Using the Mann-Whitney U-test statistic \textit{(p-value)}, we examine whether the following null hypothesis gets rejected.
\textit{Null hypothesis: The two groups under consideration have the
same distribution, i.e., a user's likelihood of making a specific decision did not change significantly (stationary)}


\subsubsection{Non-stationarity test results:}
\label{sec: tableau_non_stationarity}
We utilize the Mann-Whitney U-test for our non-stationarity analysis, splitting user interactions in half.
Under each task completed by the users, we create a separate series for each attribute, reflecting the probability of its appearance during an interaction. Non-stationarity analysis is then performed on these series to determine whether the user's interest in a particular attribute has waned, leading to its removal from their preferred list.   

The results in \autoref{fig: tableau_non_stationary} show that users are hesitant to change their preferred set of attributes in focused tasks. This is expected since the analysis tasks explicitly provided a set of attributes and asked for information related to them. Therefore, users prioritized using these attributes, resulting in a stationary decision-making policy where their preference for a particular set of attributes did not change.

Users exhibit diverse decision-making policies for goal-directed open-ended tasks (tasks T4), with both stationary and non-stationary strategies observed depending on the analysis task. For example, the goal-directed open-ended task for the weather dataset is heavily influenced by the prior focused tasks, which asked, "What weather predictions would you make for February 14th 2018, in Seattle, and why?". Most users reported findings based on previously utilized attributes from focused tasks, such as fog, mist, drizzle, temperature, and wind, rather than exploring the dataset for new attributes.
The users with non-stationary decision-making policy tried out different attributes and often added or removed attributes from their preference list.

\leilani{This subsection should have clear takeaways that naturally lead to the next sub-section (i.e., the next stage of the analysis). What are the major takeaways for the non-stationary analysis that inform the modeling of user learning? They are not clear. See the HILDA paper for example framing.}

% We perform statistical significance test among the best performing prediction algorithms.  Statistical significance, in this case the $p$-value is a more clear quantification of how close the performance of the algorithms are to each other. We used Wilcoxon signed-ranked test for statistical significance testing.
% Table \ref{tab: cb} and \ref{tab:wilcoxon} shows us that Bush \& Mosteller and No-exploration algorithm are best for predicting the users' next interaction, while adapting to the users' exploration behavior in data exploration tasks. Based on the $p-value$ of the Wilcoxon signed-ranked test we can say performance of Bush \& Mosteller and No-exploration is nearly identical $(p > 0.05)$; Bush and Mosteller being marginally better $(2\%)$. From table \ref{tab:wilcoxon} we also see that there aren't any significant difference between the performance of Adaptive $\epsilon$-Greedy and the $\epsilon$-Greedy algorithm.

% This result provides us with important insight on the nature of users' exploration behavior on current set of tasks. Performance of the baseline model (No-exploration) indicates the users' are hardly doing any exploration.+ During the user study of the Tableau interaction log the users are provided with hints for the close-ended exploration tasks. The close-ended nature of the tasks, high-dependence of the prior knowledge, users' reliance with hints, etc. explains  users' minimal requirement of exploring the dataset.
%The learned value of $\epsilon$ is $0.05$ shows that the users' are more interested in doing exploitation rather than exploration. Also, we can see that simple models such as win-keep lose-randomize are not good enough for the prediction task. We can also see that popular human learning models in economics and information searching such as, Bush and Mosteller and Roth and Erev aren't robust enough for modeling human learning in the data exploration task.\\


% Modified Roth and Erev model outperforms other models in this prediction task. But, in the open-ended task 4, the 'Bush and Mosteller' model performs similarly to the modified 'Roth and Erev' model. It even performs better than the 'Roth and Erev' for the open-ended task 4 on the birdstrikes dataset. However, considering overall prediction performance for both open-ended task 4 and close-ended task 3, modified 'Roth and Erev' is the clear winner. Table \ref{tab: ob} and \ref{tab: ow} shows the F1 score of different models on open-ended task 4. The non-learning models: random strategy and fixed strategy, which represents agents without any learning ability, performs poorly in comparison to our learning models in all scenarios.

% Prediction performance of learning models take a hit when we move from close-ended tasks to open-ended tasks.
% The number of attributes selected from the dataset is low for close-ended tasks compared to the open-ended ones.
% In close-ended tasks, the users are provided with related attribute information to find the solution, adhering to the task. Also, these tasks are simple enough to solve using those particular attributes. Therefore, the users do not need to search for new attributes; contrary to the open-ended task, where the user needs to explore the dataset to find useful attributes in order to get the desired answer. As a result, the search space for finding relevant attributes during exploration becomes a huge problem for our learning models. 
% If see the F1-score of latest reward for the close-ended tasks, it become evident that in close-ended tasks the users' keep on using similar set of attributes.
% We can also see the dismal performance of the $\epsilon-$Greedy and the adaptive $\epsilon-$Greedy algorithm. It can be contributed to the low number of interactions for the given tasks. These algorithms did not get enough runs to test all the strategies, thus unable to figure out the best ones.

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% Table [] shows the next interaction prediction accuracy of different learning models for the imMens interaction log dataset. Now, the exploration tasks given to the users' in the imMens interaction log are completely open-ended. As I discussed in the experimental settings, for the Tableau interaction dataset, our learning models has some priors based on the hints provided for the exploration tasks. Whereas, as the users' are trying to perform completely open-ended exploration without any fixed goal, the learning models do not have any priors for the imMens interaction log. The extremely low accuracy of our learning models show that for completely open-ended tasks and without any fixed goal our learning models are not able to predict what the next interaction is. The reason being in the open-ended exploration tasks, the users' do not have linear intent which makes it difficult for our linear learning models to make prediction what the next interactions will be.  
% For our experiment of predicting the next interaction we formatted our interaction log in the following way. In the Tableau interaction log, each interaction contains the attributes each user used to generate a visualization. As a result, this interaction log contains sequence of attributes, which are used in each interaction. This lets us to introduce three actions for the user: reset, adding an attribute, dropping an attribute. Now, there is another operation: replacement of attributes, which we switched with the two operations of adding an attribute and dropping an attribute. Besides as in this study, our focus is on the data processing part, so we do not focus on visualization operations.

% Current data exploration systems assume that data analysts have a fixed probability distribution for selecting a particular strategy. In other words, the likelihood of using a particular strategy remains unchanged throughout the interaction session.\\
% Research has already shown that humans show some form of learning during information retrieval tasks\cite{mccamish2018data, cen2013reinforcement}. In addition, multiple research studies on human subjects concluded that it is possible to model human-learning using reinforcement learning algorithms\cite{10.1145/1553374.1553557, shteingart2014reinforcement}.
% For our user model, it makes more sense to use reinforcement learning algorithms that adapt to change in human behavior; rather than using algorithms that learn static probability distributions for choosing each strategy. With this goal in mind, I've performed an empirical study on a real-world data exploration interaction log. Popular reinforcement learning algorithms and simple heuristics from behavioral economics, game theory, information retrieval, are evaluated to find out which mechanism closely replicates user learning. A brief description of these methods are given below.\\
% In this section, I discuss the experiments for modeling human learning in the data exploration scenario. Popular reinforcement learning algorithms and simple heuristics form behavioral economics, game theory, information retrieval are used to see which better replicates how a data analyst learns in a data exploration task. A brief description of those methods is below.
% \textbf{Latest-Reward}: The Latest-Reward method picks a strategy based on the reward that the user has seen in past interactions. Let us assume our user has $n$ strategies. By using strategy $i \in \{1, ..., n\}$, if she receives reward $r \in [0, 1]$ then the probability of picking strategy $i$ is increased by $r$. Probability mass $1 - r$ is then evenly distributed to the other strategies $j \neq i$\\
% In this experiment, the best result was obtained by setting $l = 4$, $f = 4$ for close-ended tasks and $l = 5$, $f = 4$ for open-ended tasks.\\


% Given the large action space and complexity of decisions involving multiple attributes and the prevalence of reinforcement learning (RL) for mapping human decision-making, we opted for online learning to model users' decision-making policies in this task. In online learning, the agent interacts with its environment, receives feedback (rewards or penalties), and updates its policy or value function in real-time, without the need offline training. 

==> 3_3_tableau_modeling.tex <==
\subsection{Modeling user learning}
\label{sec: tableau_user_learning}
We investigate how current human learning algorithms can adapt to the dynamic nature of IDE. With that goal, in this section, we model (inspired by existing literature) users' exploration problem in the \textit{Tableau user study} using Combinatorial Multi-Armed Bandit (CMAB), which should capture users' adaptive exploration behavior.   
% This subsection begins with an overview of the traditional Multi-Armed Bandit (MAB) problem, followed by a discussion of the CMAB problem and its relevance to the analysis tasks in our user study.
\subsubsection{Background for CMAB:}
As CMAB is a generalization of the multi-arm bandit problem (MAB), we briefly discuss these frameworks so the readers can easily relate to our exploration problem.

\noindent
{\bf Multi-Arm Bandit:} MAB problem formalizes the dilemma of acquiring knowledge about a set of K options (arms) with unknown stochastic rewards while maximizing  reward~\cite{auer2002nonstochastic}. 
The solution must learn a policy ($\pi$) that picks an arm in each try and maximizes cumulative rewards or minimizes {\it regret} over time.
The regret ($\rho$) for a policy ($\pi$) after $T$ steps, as shown in \autoref{eqn: regret}, is the difference between the sum of expected rewards for optimal policy ($\mu^{*}_{t}$) achieved by selecting the highest reward yielding arm at each time step $t \in T$, and the cumulative expected reward ($ \hat{r}_{t}$) at step $T$ for $\pi$
% current policy ($\pi$). 
\begin{equation}
    % \rho(\pi, t) = T \mu^* - \sum_{t = 1}^{T} \hat{r}_{t}
    \rho(\pi, T) = \sum_{t = 1}^{T} \mu^{*}_{t} - \mathbb{E}^{\mu}_{\pi}\bigg[\sum_{t = 1}^{T} \hat{r}_{t}\bigg]
    \label{eqn: regret}
\end{equation}

\noindent
{\bf Combinatorial Multi-arm bandit:}
In this variation of the MAB, the user can choose a subset of $n$ arms instead of selecting only one arm per time step. 
CMAB presents $n$ variables $X = \{X_1, ..., X_n\}$, where variable $X_i$ can take $K_i$ different values $\chi_i = \{v^{1}_i, ... , v^{K_i}_i\}$. The reward $R : \{\chi_1 \times ... \times \chi_i\} \rightarrow \mathbb{R}$ depends on the values of each of these variables. 
The goal of the problem is to find a vector $V \subseteq \{0, 1\}^n$ representing the subset combination of arms that minimizes the regret in \autoref{eqn: combinatorial_regret}\cite{ontanon2013combinatorial, ontanon2017combinatorial}. 
The regret equation is for policy $\pi$, where $x^{t}_1, ..., x^{t}_n$ are the values selected at time step T. 
\begin{equation}
    \rho(\pi, t) = T \mu^* - \sum_{t = 1}^{T} R(x^{t}_1, ..., x^{t}_n)
    \label{eqn: combinatorial_regret}
\end{equation}
Here, $\mu^{*} = \mathbb{E}(R(v^{*}_1, ..., v^{*}_1))$ is the maximum expected reward gained by following the optimal policy $\pi^{*}$.

\subsubsection{Modeling users' exploration problem using CMAB:}
In the \textit{Tableau user study}, users
% are presented with a sequential decision problem, where they 
select \emph{a subset of $n$ attributes}  (similar to CMAB) and perform Tableau operations to generate visualizations. 
Based on the feedback provided by these visualizations, users iterate this process until they obtain the desired information.
Through exploration, users learn to identify the ideal subset of attributes required to find their desired information, which may influence their initial exploration policy \textit{(non-stationarity: \autoref{section: ns_tableau})}. 
For instance, a user may use this new knowledge to determine if her current subset will lead her to meaningful findings.
She may modify or continue to use the same subset based on her information need \textit{(finding new information, generating new hypotheses, improving or verifying patterns, etc.)}. 
The users focus on finding the optimal subset of attributes that will generate the maximal reward, i.e., leading them to the information asked in the analysis tasks. 
% \subsection{User learning}
% In this section, we investigate whether users' learning behavior affects their decision-making policy. As discussed in \autoref{sec: tableau_non_stationarity}, the majority of the users' decision-making policies remain unchanged while completing focused analysis tasks. However, by the time they reach the open-ended task, they have learned more about the data, which has an impact on their decision-making policies. These focused tasks work as prior knowledge for the goal-directed open-ended task. Some users only use previously explored attributes to obtain the desired information in the weather dataset T4 (\autoref{sec: tableau_non_stationarity}), resulting in a stationary decision-making policy. 
% Some users leverage their learned knowledge differently; previous experience gives them time to explore other related attributes to find the desired information.

% The non-stationarity analysis results for open-ended tasks demonstrate the significant variability in users' decision-making policies when presented with the same analysis task and dataset. This difficulty highlights the challenge of proposing a generalized algorithm to model users' decision-making policies.

==> 3_3_tableau_modeling_v2.tex <==
\subsection{Formalizing user learning problem}
\label{sec: tableau_user_learning}
% \subsubsection{Modeling users' exploration problem using CMAB:}

In the \textit{Tableau user study}, users
% are presented with a sequential decision problem, where they 
select \emph{a subset of $n$ attributes}  (similar to CMAB) and perform Tableau operations to generate visualizations. 
Based on the feedback provided by these visualizations, users iterate this process until they obtain the desired information.
Through exploration, users learn to identify the ideal subset of attributes required to find their desired information, which may influence their initial exploration policy \textit{(non-stationarity: \autoref{section: ns_tableau})}. 
For instance, a user may use this new knowledge to determine if her current subset will lead her to meaningful findings.
She may modify or continue to use the same subset based on her information need \textit{(finding new information, generating new hypotheses, improving or verifying patterns, etc.)}. 
The users focus on finding the optimal subset of attributes that will generate the maximal reward, i.e., leading them to the information asked in the analysis tasks. 

Now that we aim to investigate how current human learning algorithms can adapt to the dynamic nature of IDE, we use their own objective functions for modeling purposes. 
For instance, cumulative payoff matching (PCM), a highly popular human learning algorithm in economics, has no explicit objective function. But, intuitively, they try to find action(s) / policies that will return the most payoff in the future.
On the other hand, modeling the learning problem using Multi-Arm Bandit (MAB) will enable us to use a regret minimization function to find future action(s). 
Besides using MAB variations, 

As we do not know the exact objective function a human uses during exploration, and different algorithms have different objective functions, we do not think it is ideal to evaluate the learning algorithms based on regret / cumulative reward. 

% We investigate how current human learning algorithms can adapt to the dynamic nature of IDE. With that goal, in this section, we model (inspired by existing literature) users' exploration problem in the \textit{Tableau user study}.



% using Combinatorial Multi-Armed Bandit (CMAB), which should capture users' adaptive exploration behavior.   
% This subsection begins with an overview of the traditional Multi-Armed Bandit (MAB) problem, followed by a discussion of the CMAB problem and its relevance to the analysis tasks in our user study.
\subsubsection{Background for CMAB:}
As CMAB is a generalization of the multi-arm bandit problem (MAB), we briefly discuss these frameworks so the readers can easily relate to our exploration problem.

\noindent
{\bf Multi-Arm Bandit:} MAB problem formalizes the dilemma of acquiring knowledge about a set of K options (arms) with unknown stochastic rewards while maximizing  reward~\cite{auer2002nonstochastic}. 
The solution must learn a policy ($\pi$) that picks an arm in each try and maximizes cumulative rewards or minimizes {\it regret} over time.
The regret ($\rho$) for a policy ($\pi$) after $T$ steps, as shown in \autoref{eqn: regret}, is the difference between the sum of expected rewards for optimal policy ($\mu^{*}_{t}$) achieved by selecting the highest reward yielding arm at each time step $t \in T$, and the cumulative expected reward ($ \hat{r}_{t}$) at step $T$ for $\pi$
% current policy ($\pi$). 
\begin{equation}
    % \rho(\pi, t) = T \mu^* - \sum_{t = 1}^{T} \hat{r}_{t}
    \rho(\pi, T) = \sum_{t = 1}^{T} \mu^{*}_{t} - \mathbb{E}^{\mu}_{\pi}\bigg[\sum_{t = 1}^{T} \hat{r}_{t}\bigg]
    \label{eqn: regret}
\end{equation}

\noindent
{\bf Combinatorial Multi-arm bandit:}
In this variation of the MAB, the user can choose a subset of $n$ arms instead of selecting only one arm per time step. 
CMAB presents $n$ variables $X = \{X_1, ..., X_n\}$, where variable $X_i$ can take $K_i$ different values $\chi_i = \{v^{1}_i, ... , v^{K_i}_i\}$. The reward $R : \{\chi_1 \times ... \times \chi_i\} \rightarrow \mathbb{R}$ depends on the values of each of these variables. 
The goal of the problem is to find a vector $V \subseteq \{0, 1\}^n$ representing the subset combination of arms that minimizes the regret in \autoref{eqn: combinatorial_regret}\cite{ontanon2013combinatorial, ontanon2017combinatorial}. 
The regret equation is for policy $\pi$, where $x^{t}_1, ..., x^{t}_n$ are the values selected at time step T. 
\begin{equation}
    \rho(\pi, t) = T \mu^* - \sum_{t = 1}^{T} R(x^{t}_1, ..., x^{t}_n)
    \label{eqn: combinatorial_regret}
\end{equation}
Here, $\mu^{*} = \mathbb{E}(R(v^{*}_1, ..., v^{*}_1))$ is the maximum expected reward gained by following the optimal policy $\pi^{*}$.

% \subsection{User learning}
% In this section, we investigate whether users' learning behavior affects their decision-making policy. As discussed in \autoref{sec: tableau_non_stationarity}, the majority of the users' decision-making policies remain unchanged while completing focused analysis tasks. However, by the time they reach the open-ended task, they have learned more about the data, which has an impact on their decision-making policies. These focused tasks work as prior knowledge for the goal-directed open-ended task. Some users only use previously explored attributes to obtain the desired information in the weather dataset T4 (\autoref{sec: tableau_non_stationarity}), resulting in a stationary decision-making policy. 
% Some users leverage their learned knowledge differently; previous experience gives them time to explore other related attributes to find the desired information.

% The non-stationarity analysis results for open-ended tasks demonstrate the significant variability in users' decision-making policies when presented with the same analysis task and dataset. This difficulty highlights the challenge of proposing a generalized algorithm to model users' decision-making policies.

==> 3_3_tableau_modeling_v3.tex <==
\vspace{-3mm}
\subsection{Formalizing user learning problem}
\label{sec: tableau_user_learning}
% Through interacting with Tableau, users learn to identify the ideal subset of attributes required to find the desired information.
% As we saw in \autoref{section: ns_tableau}, what they learn influences their attribute selection. 
Now we formalize the process by which users learn to find the ideal subset of attributes by interacting with Tableau to accomplish the assigned task.

Let us assume, the dataset $D$ has $n$ attributes, $D \subseteq \{a_1, a_2, ..., a_n\}$.
$X_i$ represents a user's selection of attributes at time step, $t = i$.
So, at the start of the exploration $t = 0$, $X_i = \{\varnothing\}$.
Based on our established exploration problem in \autoref{section: ns_tableau}, in each interaction $t = i$, user can take the following \textbf{actions}: 

(a) \textbf{Add one or more attributes} from set $D \setminus X_{i-1}$. 

(b) \textbf{Drop one or more attributes} from previous selection $X_{i-1}$

(c) \textbf{Keep} the same attribute set $X_i = X_{i-1}$

(d) \textbf{Reset} $X_i = \{\varnothing\}$.

The user then analyzes the visualizations generated by Tableau for $X_i$ at time step $t = i$. 
The information in these visualizations acts as a \textbf{reward} $R_i$, by which she measures the quality of the current attribute sets.
As a result, $R_i$ influences users' choice of attributes $X_{i+1}$ in the next step.
In our experiments, we gauge the effectiveness of selected attributes in accomplishing the given analysis task.
% For our experiments, we gauge the picked attributes' effectiveness and calculate reward $R_i$ by multiplying two factors: time spent at $t = i$, and quality of $X_i$.
We identify the essential attributes required for completing each analysis task, deeming them high-quality.
The effectiveness of a selected set of attributes = \#of high-quality attributes in it.  

% The quality of $X_i = \#$of high-quality attributes in it.  

% set of attributes user pick a subset of that.
% Biasness in T1 T2 towards the given attributes



==> 3_3_tableau_modeling_v4.tex <==
\vspace{-3mm}
\subsection{Formalizing user learning problem}
\label{sec: tableau_user_learning}
% Through interacting with Tableau, users learn to identify the ideal subset of attributes required to find the desired information.
% As we saw in \autoref{section: ns_tableau}, what they learn influences their attribute selection.

Given our observation of user learning during exploration, we now formalize the process by which users \textbf{learn} \textit{to find the ideal subset of attributes} by interacting with Tableau to accomplish the assigned task.
% Let us assume, the dataset $D$ has $n$ attributes, $D \subseteq \{a_1, a_2, ..., a_n\}$.
Let $X_t$ represent a user's selection of attributes at the time step, $T = t$ from the dataset $D$ with $n$ attributes.
To change her attribute preferences ($X_t$), a user may take the following \textbf{actions}: 
% So, at the start of the exploration $t = 0$, $X_i = \{\varnothing\}$.
% Based on our established exploration problem in \autoref{section: ns_tableau}, in each interaction $t = i$, user can take the following \textbf{actions}: 
(a) \textbf{Add one or more attributes} from set $D \setminus X_{t-1}$. 
(b) \textbf{Drop one or more attributes} from $X_{t-1}$
(c) \textbf{Keep} the same attribute set $X_t = X_{t-1}$
(d) \textbf{Reset} $X_t = \{\varnothing\}$.

The user then analyzes the visualizations generated by Tableau for $X_t$. 
The information in these visualizations acts as a \textbf{reward} $R_t$, by which she measures the quality of the current attribute sets $X_t$.
This process influences the subset of attributes in $X_{t+1}$, and the user gradually learns which subset of attributes will lead her to the desired information.

This problem is similar to the combinatorial bandit problem, where a user selects a subset of arms from $n$ available arms. 
In the combinatorial bandit setting, the user minimizes regret to find the optimal subset. 
But as we do not know the users' exact objective functions in IDE, for modeling user learning, we try out algorithms with different objective functions. 

In our experiments, we gauge the effectiveness of selected attributes in accomplishing the given analysis task.
% For our experiments, we gauge the picked attributes' effectiveness and calculate reward $R_i$ by multiplying two factors: time spent at $t = i$, and quality of $X_i$.
We identify the essential attributes required for completing each analysis task, deeming them high-quality.
The effectiveness of a selected set of attributes = \#of high-quality attributes in it.  

% The quality of $X_i = \#$of high-quality attributes in it.  

% set of attributes user pick a subset of that.
% Biasness in T1 T2 towards the given attributes



==> 5_1_iMens_modeling_decision_problem.tex <==
\vspace{-3mm}
\section{imMens user study}
\label{section: datasets}
\subsection{Overview of Exploration Task}
\subsubsection{imMens interaction log}
\label{section:dataset-imens}
In this user study \cite{liu2014effects} by Liu and Heer, users perform \textbf{open ended tasks} on two datasets. 
One of the two datasets has travelers' check-in data on the check-in service, \textit{Brightkite}; while the other dataset contained US domestic flight performance data \cite{liu2014effects}.
The participants are instructed to report any \textbf{\textit{interesting finding}} with a 30-minute \textbf{time restriction} per dataset, using a think-aloud protocol.
Interesting findings are defined as surprising events, data abnormalities, confirmations of common knowledge, or intuition \cite{liu2014effects}. 
The authors orient the subjects with hypothetical examples and encourage them not to be bounded by them.
Participants can quit analysis when they feel there is not anything else to discover. 
\begin{figure}[!htbp]
    \includegraphics[scale=.145]{figures/immens.jpg}
    \centering
\caption{A user exploring flight performance data using imMens. ImMens generates four linked visualizations: (1) scatter-plot: arrival and departure delays, (2) Carrier: bar chart with flight information of various US airline carriers, (3) Year: bar chart, and (4) Month: histogram with temporal information about flight time.}
\captionsetup{justification=centering}
\label{fig: immens_interface}
\vspace{-5mm}
\end{figure} 

% The authors have shared the imMens study with us,
For our work, we utilize users' raw interactions with the imMens interface, and their verbal feedback \textit{(users' explaining their actions, findings, reasonings, e.g., what type of information they want to find? If they have found anything interesting, etc.)}.

The authors ask participants to explore one of the datasets using the imMens interface with 500 ms latency to test how latency affects the IDE.
As we focus on analyzing users' exploration behavior in IDE, we only use the data from the non-latency setting. 
% The authors have shared the logs from their study with us, so we could use them for our analysis. 
% We have access to the users' raw interactions with the imMens interface in addition to their verbal feedback \textit{(users' explaining their actions, findings, reasonings, e.g., what type of information they want to find? If they have found anything interesting, etc.)}. 
% To support our analysis, we need suitable input for modeling how users learn to explore a dataset. Rather than conducting a separate user study to collect data, we observe that many visualization researchers \cite{battle2019characterizing,liu2014effects} have already conducted influential studies in this space and have publicly shared their study data.
\subsubsection{Task characteristics and learning:}
Compared to focused tasks, \textbf{open-ended tasks} provide better opportunities to track user learning, as users neither have a clear goal nor an exploration strategy.
The imMens user study gave users 15 minutes to get familiar with the dataset and interface. Such \textbf{prior experience} may impact their learning to a certain degree compared to the scenarios where users need to carry out the exploration task without any familiarity.
imMens presents \emph{linked visualizations} (\autoref{fig: immens_interface}) that participants can explore using operations: brush, pan, zoom, and range select. The set of available operations eases \textbf{task complexities} compared to complex systems like Tableau \cite{Tableau}. Additionally, imMens automatically generates visual summaries, reducing the burden on participants to determine which columns from the dataset to select to create visualizations to find relevant information.

\vspace{-3mm}
\subsection{Testing non-stationarity of user behavior}
\subsubsection{Formalizing the exploration problem:}
\label{sec: users_decision_problem}
% Users in this completely \textbf{open-ended} analysis task 
Though users may not have a predetermined strategy for selecting the order of imMens visualizations to explore, their interactions with these visualizations (\autoref{fig: immens_interface}) facilitate the learning of different aspects of the dataset.
After each interaction, the user may study one or multiple visualizations to discover information and patterns. 
Because of the \textbf{time restriction}, \textit{they quickly need to learn about the available resources in each visualization and may estimate how much information is available for extraction}. 
This sequence of interactions is modeled as an exploration problem, \textbf{where the user learns to make an informed choice about \textit{which visualization to interact with}}. 

We chronologically record the time users spend on each visualization and visualize it in \autoref{fig: time_spent_tableau}.
This illustrates that users interact with a visualization multiple times to learn about the corresponding data before switching to a different visualization. 
We also find that the distribution of time across visualizations differs as data exploration progresses.
In this section, we will see that the information users learn from visualizations, combined with their \textbf{past experiences}, influence their choice of exploration policy, i.e., which visualizations to interact with over time. So, \textit{users must decide: (a) which visualization to pick (b) continue focusing on a specific visualization for more information (c) switching to a different visualization in hope of more/interesting information.}
% This decision varies depending on whether they believe they have already exhausted all the information from the current visualization, there may be interesting patterns to discover in other visualizations, or whether they want to verify their recent insights using other data areas.
% For example, the visualization users favor in the first half of their exploration session is rarely the same visualization that they focus on in the second half.
\\
\noindent
\textbf{Example: }\emph{Participants sequentially clicked on different carriers (from the visualization `Carrier' in \autoref{fig: immens_interface}) in search of patterns}. 
As users learned more about the data, their exploration behavior evolved.
For instance, \emph{some users noticed a surge of new airlines in 2003 from the visualization `Year', and rather than focusing on random carriers, they investigated those introduced in 2003}. 

Learning about the data enables users to prepare an exploration policy regarding which data regions to analyze. As they learn more, they can refine their policy accordingly.  
\begin{figure*}[!htbp]
    \includegraphics[width = \textwidth]{figures/time_spent_tableau.jpg}
    \centering
\caption{Users' focusing on different visualizations during imMens exploration task}
\captionsetup{justification=centering}
\label{fig: time_spent_tableau}
\end{figure*} 
\label{sec: imMens_decision_problem}

\subsubsection{Mann Whitney non-stationarity test:}
\label{subsec: iMens_nonstationarity}

We analyze changes in users' exploration policies across all visualizations to test our hypothesis that user learning influences exploration policy. 
% \FloatBarrier
% \vspace{-3mm}
% \subsubsection{Non-stationarity test}
We divide each participant's exploration session with the flight performance dataset into two partitions, $S_1$ and $S_2$. 
Then we generate the exploration policy, i.e., the probability of interacting with each visualization. 
% We chose to use a 50-50 split, as it represents the most fundamental level at which we would expect to observe changes in strategy.
% Four visualizations are presented by imMens for the flight performance dataset, which are $A_k, k = \{1, 2, 3, 4\}$, and the user made \textit{n interactions} $I_{k}$, $k \in \{1, ..., n\}$. For each user, we create subtask 1, $S_1 = \{I_{i}\}, i = \{1, ..., floor(n/2)\}$ with the first half of the imMens interactions, and the rest going to subtask 2, $S_2 = \{I_{i}\}, i = \{floor(n/2) + 1, ..., n\}$. For each subtask, we generate a series of numbers $P_i(A_k | I_i) \in [0,1]$ where $I_i \in \{S1, S2\}$. We generate such series for each visualization(arm) $A_k$ where $P_i$ refers to the probability of a visualization $A_k$ being picked at interaction $I_i$.
% We then use the Mann-Whitney U test to compare the decision-making policies $\pi(A_k)$ at different stages of the data and detect any changes in the policies (i.e., probability of selecting a visualization). If such changes occur, we can conclude that the users' decision-making policy is non-stationary.
% \subsubsection{Non-stationarity test using Mann-Whitney}
We perform a Mann-Whitney U-test \cite{mcknight2010mann, mann1945nonparametric} on each visualization using $S_1$ and $S_2$ to determine if these probability series are significantly different (\textit{non-stationary}). 

\emph{\autoref{fig: ns_50_first}(a) shows that the distribution of visualization selection is mostly non-stationary} ($81.25\%$).
The test results align with our analysis of \autoref{fig: time_spent_tableau} in \autoref{sec: users_decision_problem}. Users learn about information available in each visualization and change their exploration policy, i.e., engage in non-stationary exploration, as relying on a single visualization would be sub-optimal.
% \vspace{-3mm}
\begin{figure}[!htbp]
\centering
\includegraphics[scale=.3]{figures/imMens_NonStationarity.png}
\caption{For each user and visualization, we see significant non-stationary behavior between $S_1$ \& $S_2$}
\label{fig: ns_50_first}
% \vspace{-3mm}
\end{figure}

% \subsubsection{Non-stationary multi-arm bandit:}
% \label{subsubsection: mba} 
% In this variant of the multi-arm bandit problem, there are $K$ arms, and the reward distribution for each arm changes over time. This is in contrast to the standard multi-arm bandit problem, where the reward distribution for each arm remains constant.
% The agent's goal is to learn a policy ($\pi$) that minimizes regret (or maximizes cumulative rewards) over time, adapting to the non-stationary nature of reward distribution.

% The regret ($\rho$) for a policy ($\pi$) after $T$ steps, as shown in \autoref{eqn: regret}, is the difference between the sum of expected rewards for optimal policy ($\pi^{*}$) achieved by selecting the highest reward yielding arm at each time step $t \in T$, and the cumulative expected reward at step $T$ for policy ($\pi$). 
% Here $\mu^{*}_{t}$ is the maximum expected reward at time step $t$ for optimal policy.
% \begin{equation}
%     % \rho(\pi, t) = T \mu^* - \sum_{t = 1}^{T} \hat{r}_{t}
%     \rho(\pi, T) = \sum_{t = 1}^{T} \mu^{*}_{t} - \mathbb{E}^{\mu}_{\pi}\bigg[\sum_{t = 1}^{T} \hat{r}_{t}\bigg]
%     \label{eqn: regret}
% \end{equation}
% % The MAB problem assumes a stationary reward distribution, but when it changes over time, it becomes a non-stationary multi-arm bandit problem. 
% In non-stationary cases, recent rewards are more important than long-term rewards. Popular approaches to tackle this temporal uncertainty include using a constant step-size  parameter\cite{auer2002nonstochastic, garivier2008upper} and assigning a lifetime to each bandit\cite{chakrabarti2008mortal}.
% The step-size approach tracks changes in an arm's reward distribution after $n$ pulls, while the lifetime approach assumes that the arm will expire after $n$ pulls.

% \subsubsection{Modeling the decision problem using non-stationary MAB}
% \label{sec: imMens_decision_problem}
% In our decision-making problem, the user is presented with \textit{$K$ visualizations}, and at each time step, the user can pick one visualization similar to pulling an arm.  
% Because of the time constraint, users aim to maximize the reward they receive, making each interaction worthwhile.
% Due to the finite amount of information in each visualization, relying solely on a single visualization that has yielded maximum information in the past can lead to sub-optimal results. Switching to a different visualization after extracting sufficient information from the current one changes the reward structure and thus makes the decision problem non-stationary. We can associate a lifetime with each visualization asserting that after that time, it loses its importance as an information source for a user. 

% \subsubsection{Notion of reward in our decision-problem:}
% Users receive rewards by interacting with each visualization in the form of information. A reward $R \in (0,1]$ is assigned to imMens interactions at each time step, $t$, depending on their usefulness for finding information. A reward of $R = 0.1$ is awarded to an interaction for making a simple observation. On the other hand, making generalizations, creating questions or hypotheses, confirming hypotheses, and finding answers lead to reward $R = 1$. We assign higher rewards in these circumstances, as these interactions propel users' data exploration. For example, generating a hypothesis (question) leads to interactions to find desired information and instigates users to find new information or patterns. Interactions that do not lead to any information receive a reward of $R = 0$. Each user tries to maximize the amount of information by minimizing regret (\autoref{eqn: regret}) over 30 minutes.
% Detecting changes in user behavior using low-level raw actions is extremely hard. Information demand, interface, data, and other factors influence these actions. 
% We need to comprehend users' information needs in order to determine how they are evolving (during exploration). 

% The \textit{imMens user study} had participants explore flight performance and travel history data to uncover interesting insights, such as unexpected events, data abnormalities, or confirmations of common knowledge and intuition. 
% Each participant had a maximum of 30 minutes to examine a single dataset and could terminate the session early if they felt there was nothing noteworthy to report. \cite{liu2014effects} 

% One dataset included 4.5 million user check-ins over 2-years period on a location-based check-in service, \textit{Brightkite} \cite{cho2011friendship}. 
% Other contained on-time performance data of US domestic flights from 1987 to 2008, comprising 140 million records \cite{FAA1}.

% Liu and Heer conducted a user study~\cite{liu2014effects} to understand how analysts change their exploration behavior when they experience \emph{latency} in the user interface. They recruited 16 analysts who used imMens~\cite{liu2013immens} \textit{(a tool that enables visual exploration of large datasets)} to explore two datasets.

==> 5_3_iMens_user_learning.tex <==
\subsection{User learning}
\label{sec: iMens_userlearning}
As discussed in \autoref{subsec: iMens_nonstationarity}, the results show a shift in users' decision-making policy in the \textit{Tableau user study}. In this section, we investigate whether users' learning behavior during data exploration played a role in inducing this change.
The participants were presented with new datasets and therefore did not have prior knowledge of which visualization to prioritize when imMens suggested visualizations for information extraction. 
We can see from \autoref{fig: immens_interface} that the visualizations act as different sources for information and patterns. For example, the \textit{Scatterplot} visualization shows the relation between arrival delay and departure delay on a 2D plane. The visualization \textit{Carriers (bar-chart)} contains flight information of various US airline carriers. And \textit{Year (bar-chart)} and \textit{Month (histogram)} contains temporal information about the time these flights took place. 

Due to time constraints and the non-stationary nature of the exploration problem, users must make informed choices about which visualizations to interact with. Through interacting with each visualization, they learn about available resources and can estimate what information are available for extraction. For example, \emph{participants sequentially clicked on the carriers shown in the visualization carrier and looked for patterns}. As users learned more about the data, their decision-making policies changed. For instance, \emph{some users noticed a surge of new airlines in 2003 from the visualization year, and rather than focusing on random carriers, they investigated those introduced in 2003}. Gaining knowledge about the data lets users prepare an exploration policy on which data areas to look at. For example, \emph{some users focused solely on carriers with a high number of flights, while others found those with a low number of flights intruiging}.     

Users' learning impacts their exploration strategy as they decide which data area to explore next. For instance, when interacting with different carriers (carriers), some users find patterns and make observations from the spatial data (scatterplot) or temporal data (year, month). These observations influence their choice of future visualization to explore once they have exhausted the visualization \textit{carrier}.

% The users also learn when to switch their focus to a different visualization to maximize their accumulated reward. As we discussed, sticking with a visualization that yielded lots of information in the past may not remain the optimal choice for future stages of data exploration. And from the results of \autoref{fig: ns_50}, we can see that users are doing exactly that. Rather than sticking with an optimal arm (visualization), the users are changing their focus to different visualizations to maximize their accumulated reward. This also explains why the users display non-stationary behavior during data exploration. 
% Not to mention information available in a particular visualization might be limited or require additional information from other visualizations. 
% Which is clear from our experiment results in \autoref{fig: ns_50_reward}. We used the Mann-Whitney U-test on partition $S_1$ and $S_2$ to check if an arm (visualization) always yields reward from the same distribution. We can conclude from the  results in \autoref{fig: ns_50_reward} that the reward distribution changes significantly in the second half of our decision making problem.

==> 5_3_imMens_modeling_v2.tex <==
\vspace{-3mm}
\subsection{Modeling user learning}
{\bf Multi-Arm Bandit:} MAB problem formalizes the dilemma of acquiring knowledge about a set of K options (arms) with unknown stochastic rewards while maximizing  reward~\cite{auer2002nonstochastic}. 
The solution must learn a policy ($\pi$) that picks an arm in each try and maximizes cumulative rewards or minimizes {\it regret} over time.
The regret ($\rho$) for a policy ($\pi$) after $T$ steps, as shown in \autoref{eqn: regret}, is the difference between the sum of expected rewards for optimal policy ($\mu^{*}_{t}$) achieved by selecting the highest reward yielding arm at each time step $t \in T$, and the cumulative expected reward ($ \hat{r}_{t}$) at step $T$ for $\pi$
% current policy ($\pi$). 
\begin{equation}
    % \rho(\pi, t) = T \mu^* - \sum_{t = 1}^{T} \hat{r}_{t}
    \rho(\pi, T) = \sum_{t = 1}^{T} \mu^{*}_{t} - \mathbb{E}^{\mu}_{\pi}\bigg[\sum_{t = 1}^{T} \hat{r}_{t}\bigg]
    \label{eqn: regret}
\end{equation}

\noindent
\textbf{Non-stationary multi-arm bandit:}
We've already introduced traditional MAB in \autoref{sec: tableau_user_learning}. 
Users' strategy for exploring the flight performance dataset using imMens can be considered a MAB problem; the user is presented with \textit{$K$ visualizations}, and at each time step she can pick one visualization similar to pulling an arm. 
The user must then learn a policy that maximizes the information received by interacting with visualizations over time.
% However, in the traditional MAB, each arm has a fixed reward distribution.
However, in real-life scenarios, reward distribution rarely stays stationary and requires modeling the learning problems as non-stationary MAB \cite{chakrabarti2008mortal, besbes2014stochastic, cavenaghi2021non}.
Similar to these research, in our problem, the amount of interesting information users can gain from each visualization might decrease after a while.
Users may switch to a different visualization after extracting sufficient information from the current one or use multiple visualizations to acquire the necessary information, which alters the reward structure of each visualization.
%users learn to change their exploration policy as they switch visualizations to gather more knowledge (\autoref{sec: iMens_modeling}). 
%However, relying solely on a previously informative visualization during exploration may be sub-optimal due to finite information. 
To address this issue, we model users' learning problem as a variant of the standard MAB, \textit{Non-stationary} MAB, where the arm-reward distribution changes over time \cite{chakrabarti2008mortal}.

\noindent
{\bf Visualization Reward:} Users receive rewards by interacting with each visualization in the form of {\it information}. 
We assign reward $R \in [0,1]$ to each interaction, depending on its usefulness for finding information. 
We set the reward of an interaction that generate \emph{simple observation} to $R = 0.1$. 
On the other hand, \emph{making generalizations, creating questions or hypotheses, confirming hypotheses, and finding answers} lead to reward $R = 1$. 
We assign higher rewards in these circumstances, as these interactions propel users' data exploration. 
For example, generating a hypothesis (question) instills users to find new information or patterns. 
Interactions that do not lead to any information receive zero reward. 
Each user tries to maximize the amount of information by minimizing regret (\autoref{eqn: regret}) over 30 minutes.

% To design a data exploration system that can adapt to users'
% information needs throughout their learning process, the system must anticipate their choice of exploration policies based on their learning behavior. 
% In this section, we model user learning and test popular algorithms from existing research in modeling human learning.
% In this section, we first briefly explain the non-stationary variant of the MAB introduced in \autoref{sec: tableau_user_learning}, followed by a discussion on how we model user exploration policies using this framework. 


==> 5_4_iMens_algorithms.tex <==
\subsection{Evaluated learning algorithms}
\begin{comment}
\subsubsection{Multi-Arm Bandit (MAB):}
In this problem, there is a K-arm bandit machine with unknown stochastic rewards ~\cite{auer2002nonstochastic}. 
In each round, an agent can pull one arm and receives some reward.
The agent's objective is to learn a policy ($\pi$) for picking arms optimally that minimizes {\it regret} over time.
\autoref{eqn: regret} shows the regret ($\rho$) for policy ($\pi$) after $T$ steps, which is the difference between the sum of expected rewards for optimal policy ($\mu^{*}_{t}$) achieved by selecting the highest reward-yielding arm at each time step $t \in T$, and the cumulative expected reward ($ \hat{r}_{t}$) at step $T$ for $\pi$
% current policy ($\pi$). 
\begin{equation}
    % \rho(\pi, t) = T \mu^* - \sum_{t = 1}^{T} \hat{r}_{t}
    \rho(\pi, T) = \sum_{t = 1}^{T} \mu^{*}_{t} - \mathbb{E}^{\mu}_{\pi}\bigg[\sum_{t = 1}^{T} \hat{r}_{t}\bigg]
    \label{eqn: regret}
\end{equation}

\noindent
\textbf{Non-stationary MAB:}
However, in real-life scenarios, reward distribution rarely stays stationary and requires modeling the learning problems as non-stationary MAB \cite{chakrabarti2008mortal, besbes2014stochastic, cavenaghi2021non}.
\vspace{-2mm}
\subsubsection{Modeling user learning as non-stationary MAB:}
% We consider the \textit{$K$ visualizations} as K arms, where at each round, the user picks a visualization to analyze, similar to pulling an arm. 
We consider the \textbf{\textit{K visualizations} as a K-arm bandit} machine, where instead of an arm pull, the user picks a visualization to analyze.
The user receives information after she completes an imMens operation on the selected visualization.
This information acts as a {\bf reward} that influences the user's choice of future visualizations.

The static nature of the given dataset implies that information within a specific data area remains constant.
As a result, the more a user analyzes a visualization and reports her interesting findings, the less likely she is to discover new information.
Considering the user's goal in exploring data is to find interesting information, based on our learning problem, her policy of choosing visualization may change.
This adaptation influences the reward structure of each visualization, leading us to consider the reward distribution non-stationary. 
Thus, we employ a non-stationary MAB approach.

This formalization enables us to use algorithms like Mortal-Arm Bandit, which allows us to assign a lifetime to each visualization (arm).
After a lifetime of pulls, a user would consider the visualization dead and switch to other arms for more rewards.
In our case, users may revisit the same arm multiple times during IDE, so we introduce the killed visualization as a new visualization.
\end{comment}

\label{sec: algorithms-openended}
We use learning algorithms to model users' decision-making policies in \autoref{sec: imMens_decision_problem}. 
To balance the exploration-exploitation trade-off in this domain, we employ $\epsilon$-Greedy, $\epsilon$-Greedy with $\epsilon$ decay, and adaptive $\epsilon$-Greedy algorithms. We also compare these algorithms to win-stay-lose-shift and greedy approaches. Further details on these algorithms are available in \autoref{sec: tableau_methods}.

\noindent
\textbf{Mortal-arm bandits:} Chakrabarti et al.\cite{chakrabarti2008mortal} introduced the concept of mortality, where each arm $(i)$ has a finite lifetime ($L_i$). 
The authors propose two mortality implementations: \textit{budgeted death}, where each arm dies after $L_i$ selections drawn from a geometric distribution with an expected budget of $L$, and \textit{timed death}, where each arm dies with probability $p$ and have a lifetime of $L=1/p$. 
Originally used in the online-advertising setting, the algorithm's objective is to maximize the expected total reward by selecting an optimal sequence of arms to pull. 
After an arm's death, it is removed from the pool of available arms and a new arm can replace it. 
So, the pool size $K$ remains constant. 
The authors propose a state-oblivious algorithm for mortal-arm bandits,  
% with stochastic reward distribution. 
where instead of pulling each arm once to estimate the payoff, each arm is pulled $n$ times and abandoned if deemed unpropitious. 
% It is also perfect because of the time constraint on our analysis task.

\noindent
{\bf Evaluation Process:} 
To account for potential variations in user learning during different stages of data exploration, we assess the algorithms using varying amounts of training data. 
Using user interaction data within specific thresholds, we identify optimal hyperparameters and train the algorithms accordingly.
We evaluate how well these algorithms can predict users' future actions \emph{(i.e., which visualization the user will use in the subsequent interaction)}.

% \subsection{Experimental settings}
% \label{sec:experiment-procedure}
% \subsubsection{Hyper-parameter Tuning}
% We test the accuracy of these algorithms on our users. Adaptive $\epsilon-$greedy has hyper-parameter $l, f$, and $\epsilon-$greedy, $\epsilon-$greedy with decay parameter has hyper-parameter $\epsilon-$. Mortal arm-bandit has a parameter $L$, lifetime of the arms. To optimize our models' hyper-parameters and ensure its efficiency, we utilize a distinct percentage of the available data for training and tuning the model. Following this, we evaluate the performance of the algorithms on the remaining data. In the subsequent section, we will investigate how the size of the training data affects the performance of the algorithm, and analyze the impact of this variable on these models overall accuracy and effectiveness. 

% \subsubsection{Model training methodology:}
% As we have established in previous sections that learning is a gradual process that occurs over time and experience, we defined training thresholds to capture this , ranging from a lower limit(users are done learning early on) of 10$\%$ to an upper limit(still learning till the end) of 90$\%$ of all user interaction data. For each of these training thresholds, we determine the optimal hyper-parameters for all algorithms. We then training the models with the determined hyper-parameters on the user's interaction data within each threshold range. Finally, we test each of our models confirmation of user behavior in testing data.



==> 5_5_iMens_results_discussions.tex <==
\begin{figure}[!htbp]
\centering
\includegraphics[scale=.47]{figures/accuracy_aggregated.png}
% \includegraphics[width=\textwidth]{figures/accuracy_aggregated.png}
\caption{Accuracy of different algorithms after being trained on different percentage of data, using flight performance dataset exploration interactions}
\label{fig: accuracy1}
\end{figure}

\label{sec: results_immens}
\begin{figure}[!h]
\centering
\includegraphics[scale=.38]{figures/Performance-Metric.png}
\caption{Performance of discussed bandit algorithms. Comparison of reward obtained by these algorithms w.r.t. the reward obtained by a user.}
\label{fig: regret}
\end{figure}
\subsection{Performance evaluation}
\label{fig: imMens_results}
\subsubsection{Evaluation methodology:}
In this section, we evaluate state-of-the-art learning algorithms \autoref{sec: algorithms-openended} for modeling participants' decision-making policy in an open-ended analysis task, using non-stationary multi-arm bandits, as described in \autoref{sec: iMens_modeling}. 
Here, we evaluate the algorithms' ability to predict users' future decisions, which depends on their capability to adapt to changes in the decision-making policy. By assessing their prediction capability \emph{(i.e., which visualization the user will use in the subsequent interaction)}, we can evaluate the effectiveness of the models in adapting to changes in the users' decision-making policies.

\subsubsection{Results and discussion:}
Contrary to our previous studies (\autoref{sec: tableau}, \autoref{sec: forecache}), we observe different results for \textit{completely open-ended analysis tasks}. The figures in \autoref{fig: regret} and \autoref{fig: accuracy1} indicate that it is challenging for learning algorithms to model users' non-stationary decision-making policies in such scenarios. 

Win-Stay-Lose-Shift (WSLS) policy outperforms others with 60\% average prediction accuracy, followed by $\epsilon$-Greedy and $\epsilon$-Greedy with $\epsilon$ decay with ~52\% accuracy. WSLS works well since users spend a significant amount of time in a particular visualization, as seen in \autoref{fig: time_spent_tableau}. 
However, this heuristic falls short in detecting changes in users' decision-making policy, which is crucial for our purpose of modeling it. It relies entirely on the failure of a decision to correct its course by randomly choosing a decision, which can take some time.

On the other hand, the $\epsilon$-Greedy and $\epsilon$-Greedy with $\epsilon$ decay algorithms fail to adapt quickly to changes in users' decision-making policies due to the open-ended nature of the analysis task. How long a user interacts with a particular visualization varies throughout the exploration session, which makes it difficult to determine the appropriate hyper-parameter values. Additionally, users may not need to revisit a previously exhausted visualization.

Adaptive $\epsilon$-greedy and mortal bandit algorithms face the same limitation due to their reliance on hyper-parameters, step size, and lifetime, resulting in poor performance. Despite being designed for non-stationary multi-arm bandit problems, users' exploration policies do not strictly follow these hyper-parameters during the exploration session.   

==> 6_common_results_old.tex <==
%better name for this section: spend more time. Should have 2 sub-section, 1)What we have found 2)Connect these findings to characteristics
%2) How these findings may influence designing interacting systems. Example: the need for non-stationarity-based systems rather than offline training/fixed system/stationary systems.
\section{Discussion}
\label{sec: discussion}

We identify common themes across the three user studies we analyzed our (\autoref{tab:user_study_high_level}), which we use to summarize our community's current understanding of how users learn during data exploration versus how this learning is modeled in practice. Based on these findings and our own experiences, we suggest future research directions in developing more accurate models of user learning and exploration as well as learning-aware data exploration systems.
%We summarize common findings from our evaluation of state-of-the-art algorithms on the three user studies (\autoref{tab:user_study_high_level}) and discuss the observed characteristics of user learning and share \textit{our learnings} that propel application-driven considerations for the design and modeling of user learning.

% We have empirically analyzed user learning behavior in diverse analysis tasks, differing by the characteristics introduced in \autoref{sec:charactetistics_of_exploration_task}, using non-stationarity tests.
% In this section, we summarize our findings on how these characteristics influenced users' learning behavior and impacted their strategies chosen during data exploration. 
% Additionally, we generalize our findings of the modeling process of user learning behavior using online learning algorithms and how users' diverse behavior made it difficult. Furthermore, we discuss the benefits of user learning models in designing interactive data exploration systems.

\subsection{Characteristics of user learning}
\noindent
\textbf{Exploration task characteristics} influence user learning and thereby users' exploration strategies.
% \leilani{Who is being referred to in ``their strategies''?}
 We find that if users have \textbf{prior experience} \textit{actively solving} tasks at the same level of \textbf{complexity} as the current task (\autoref{sec:tableu_perfromance_evaluation}), they may not be sufficiently challenged to learn. 
 On the other hand, \textit{simply familiarizing} users to the dataset and interface prior to the task may not significantly hinder learning during the actual task(\autoref{sec: forecache_results}).
 These findings resonate with research by Csikszentmihalyi et al~\cite{csikszentmihalyi2014flow}, suggesting that observing true learning-directed exploration may require participants to enter a flow state(mental state) that balances the user's prior experience with what is being asked of them (task challenge level), otherwise learning may not occur within the controlled lab environment. 
% \leilani{Should the previous sentence say inhibit? Will the complex pre-task help or harm learning? I'm confused.}
We also find that the user learning schemes' are correlated with the level of \textbf{open-endedness} of the task. For instance, Win-Stay-Lose-Shift exhibits contrasting performance between completely open-ended task in \autoref{sec: imMens_results} and the other two tasks in \autoref{sec:tableu_perfromance_evaluation} and \autoref{sec: forecache_results}. 
% \leilani{I'm not sure what is being referred to with the term ``exploration need''. Can you clarify?}\\
%seems like we have changed exploration need to 'open-endedness' 

% \leilani{The above paragraph makes me think of Mihaly Csikszentmihalyi's research in flow states. Basically, a flow state is achieved when someone is performing a task that is at the perfect level of challenge, which requires a balance between the difficulty of the task and the user's experience with the task. It might be useful to mention this concept above. For example: observing true learning-directed exploration may require participants to enter a flow state that balances the user's prior experience with what is being asked of them (task challenge level), otherwise learning may not occur within the controlled lab environment. This suggests that to study learning, exploration tasks may need to be customized to each participant's prior experience and perception of the task difficulty. To avoid this additional work, an alternative option is to carefully recruit participants at a certain level of expertise so the same task can be used across participants.}

\noindent
\textbf{Learning schemes} vary across users, based on individual differences in prior knowledge and cognitive abilities, but there may exist algorithms that best represent an \textbf{average user's learning}. For instance, among the 7 algorithms evaluated in ForeCache user study (\autoref{sec: forecache_results}), Reinforce, Actor-Critic and Greedy sufficiently capture all users' learning, and even among these three, Reinforce is the top learning scheme for 70\% of the participants.
% \leilani{I'm confused, is it all users or is it 70\% of users?}
% Reinforce is top for 70a\% of the users 
Additionally, our findings For instance, Reinforce performs better than the more complex Actor-Critic in \autoref{sec: forecache_results}, and Greedy performs very close to Bush $\&$ Mosteller in \autoref{sec:tableu_perfromance_evaluation}. Similarly, simple heuristics, such as Win-Stay-Lose-Shift, perform better than other complex algorithms in \autoref{sec: imMens_results}. %\leilani{This is a very nice result!}
 
% The diverse characteristics of our data exploration task, \textit{instructions, goals, complexity, and prior knowledge}, depict their influence on users’ decisions to change policies during exploration. In this section, 

% \textbf{Sub-optimal Learning}: When users complete a task quickly,a suboptimal but effective solution exists based on \textit{cognitive load}. For instance, focused tasks with lower cognitive load and clear analysis goals (or precise information needs) require short completion times. The concise task requirements guide user's exploration making sub-optimal learning models (such as greedy algorithm) sufficient to predict user exploration policies.


%Therefore, starting with simple algorithms is better than getting lost in the complexities of hyper-parameters and other model choices. 
%This finding supports our choice of simple human learning algorithms from cognitive and neuroscience literature.
% When designing a robust interactive data exploration system, we should be aware of their shortcomings in critical scenarios (e.g., concept drift for more adventurous users). 

\subsection{Challenges to design a user learning model}
We observe one key shortcoming of existing algorithms in adapting to user learning behavior during data exploration: they fail to anticipate user behaviors under completely \textbf{open-ended exploration} tasks.
%Specifically, current algorithms are challenged most when exploration is completely \textbf{open-ended}.
%For instance, in our evaluation of the imMens task (\autoref{sec: imMens_results}), while intuitively we expect user's to learn \textit{(algorithms performance to get better)} with more experiences \textit{(training data)}, we find such is not necessarily the case.
For example, we expected the tested algorithms to improve in performance with successive training data, similar to how analysts in the imMens study learned from new experiences  (\autoref{sec: imMens_results}). However, this was not necessarily the case.
Without any direction from pre-defined task objectives, users' exploration strategies are extremely non-stationary (\autoref{subsec: iMens_nonstationarity}) suggesting that users' learning algorithms themselves may also be evolving. As a potential solution to this challenge, we propose training an ensemble of models for user learning in complex data exploration tasks. In this way, the system can pivot gracefully when the current model fails to capture the user's learning behavior.
% % Why are our exploration-exploitation algorithms falling short in capturing users' exploration behavior to a greater extent? The answer is \textit{sequential} nature of exploration in these analysis tasks.
% In this paper, we establish the shortcomings of existing state-of-the-art algorithms in adapting to user learning behavior in complex tasks like data exploration. It is expected that none of the algorithms can perfectly capture user learning, because the decision problem is a high-level abstraction of the user's logged interactions. There are multiple features that can be considered, including but not limited to \textit{data features} like low-level interactions, planning time, and \textit{task features} like, time allocation, the extent of cognitive load, and weight of prior knowledge. There is a necessity for feature-dense and well-tuned learning algorithms that can better model human learning.

% % In this paper, we establish the shortcomings of existing state-of-the-art algorithms in adapting to user learning behavior in complex tasks like data exploration. And we discuss the necessity of feature-dense and well-tuned learning algorithms that can better model human learning.

% The exploration-exploitation algorithms covered in this article make the assumption that an agent first chooses actions at random, but as she gains experience, she continues to use actions that produce high rewards. Additionally, the agent periodically selects actions randomly to discover potential high-reward actions.
% Whereas during sequential data exploration, users engage in an exploration-exploitation cycle. Here, they explore a data area and keep exploiting it for information; until they determine its usefulness. They then move on to a new data area and repeat the cycle, extracting all relevant information until they are satisfied with their findings to solve the given task.

% The models face challenges in detecting when users switch from exploration to exploitation without any external signal. Additionally, due to concise exploration behavior, the algorithms do not receive enough interactions to accurately predict the user's next action from a large action space, especially considering hints and prior knowledge.
% This highlights the need for models to adapt to the pivot point and improve the performance of exploration-exploitation algorithms. 


\subsection{Application considerations of user learning}
\textbf{Existing user studies or new designs}: We use established studies of data exploration from the visualization and HCI communities (\autoref{tab:user_study_table}) to model learning.
%Our research did not necessitate a self-designed, `user-learning-targeted' study because such a tailored study would provide little support to our assertion that \textit{learning is natural to most general data exploration tasks}.
The diversity of selected studies, coming from multiple scholarly works, provided an opportunity to observe, formalize, and model diverse users and their learning behaviors.
Further, these works span the gamut of definitions for data exploration, allowing us to rigorously test our hypotheses amid competing definitions.
Finally, as Zgraggen et al. observe~\cite{zgraggen2018investigating}, users rarely have the awareness nor the desire to detail the ground truth of everything they learn during exploration. As a result, conducting a new user study would not yield significantly better results than those of established studies. Instead, we aim to model user learning from a diversity of regarded perspectives from the visualization and HCI community.
That being said, data exploration systems do not yet account for user learning, revealing opportunities to \emph{observe how analysts respond to learning-aware systems} in future studies.
%Additionally, we built on these prior researches to better understand the factors influencing user behavior (\autoref{tab:user_study_high_level}).  However, self-designed studies with the same population across tasks may be considered to reduce variance based on user characteristics, including the weight of prior knowledge and  cognitive abilities. Such user studies may lack the comprehensiveness of our analysis but can help build low-variance baseline models and make early experiments less overwhelming.
%having same users across tasks can help analyze differences in the users' exploration strategies between tasks.
%However, \textbf{Currently, many user studies try to discount learning cite..}; therefore, self-designed user studies may be considered. 
%if the research goal is to test the impact of one task over another. For example, in \autoref{sec:tableau_task_charactertistics}, we find focused task serves as prior experience to goal-directed open-ended tasks.

\noindent
\textbf{Premodelling decisions:} Premodelling steps, such as correct \textit{decision problem formulation} and testing for \textit{non-stationarity} behavior, are foundational to the choice of user learning models. For example, if users exhibit stationary exploration strategies, no learning may exist to be modeled. Similarly, formalizing the user's learning problem with standard MAB/MDP or their variations depends on the nature of the exploration tasks: are users' decisions independent? Or is there clear sequential dependence between state transitions?







==> 8_conclusion.tex <==
\section{Conclusion and future work}
We present a framework to formalize, quantify and model user learning. We utilize this framework to analyze user learning in diverse real-life data exploration tasks. We present the impact of the characteristics of exploration tasks on the performance of state-of-the-art online learning models. Finally, we discuss the shortcoming of current approaches and share \textit{our learnings} that propel application-driven considerations for the design and modeling of user learning. 


We plan to build an {\bf learning-aware data exploration system} that leverages a user learning model to predict users' exploratory actions. We propose two directions for our \textit{online} system design: the system may start with an initial, generic, and potentially inaccurate model and improve the model over time or have an ensemble of models trained over the course of initial interactions. The system will then choose the most accurate one after a sufficient number of interactions. We believe that such system would also provide new research directions towards understanding {\bf user's acceptance of learning-aware systems}

% Through extensive user study we aim to show using such adaptive learning model will give an interactive  
% considering analysts' exploration behavior is changing and using our learning model will give interactive data exploration system that considerable edge over the state-of-the-art systems

% To aid data analysts' in exploration tasks, we need to understand their exploration behavior. 
% Modeling their behavior can have multi-faceted benefits, such as identifying interesting data locations, providing action suggestions for high-quality exploration, and prefetching data to improve interactivity. Which will provide the analysts with an effective and efficient data exploration experience. But studying human behavior is a challenging endeavor.
% Especially in a complicated domain like data exploration, where analysts are frequently confronted with new datasets and exploration tasks. As we've discussed, data analysts' exploration behavior evolves as they get more accustomed to the interface and gain more knowledge about the data. Current user behavior modeling attempts are interface and data-agnostic. However, due to the evolving nature of user strategies during data exploration, a general yet robust model must be built. In our future works, we aim to propose a learning model that adapts to the exploration and learning behavior of data analysts, designing an interactive data exploration system that outperforms state-of-the-art systems by taking advantage of that model. 
% data exploration is not a domain
% how to model 
% how to adapt to this model this behavior
% what to do in the conference paper 
% more studies
% much shorter
% do user strategies evolve over-time in open-ended data exploration 
% Predicting user behavior and assisting users in finding information quickly and efficiently are significant aspects of today's interactive data analytics platforms. It can be accomplished in a variety of ways,  However, presuming that users' exploration strategies converge to a given probability limits the system's potential and applications. 
% We plan to solve this issue in the future by proposing learning models that mirror the exploration and learning behavior of data analysts. We also aim to show how effective such models are.

% Current user behavior modeling attempts are interface and data-agnostic. However, due to the evolving nature of user strategies during analytics, a general yet robust model must be built on mixed-initiative systems for data exploration.   

%\section{Conclusion}
%In this paper, we show that data analysts exhibit non-stationary exploration behavior in real-world data exploration tasks using the Mann-Kendall statistical trend test. Considering data analysts' change their exploration strategy, will benefit in designing better interactive data exploration solutions. 
